Revisiting the Performance of Deep Learning-Based Vulnerability Detection on Realistic Datasets

The impact of software vulnerabilities on everyday software systems is significant. Despite deep learning models being proposed for vulnerability detection, their reliability is questionable. Prior evaluations show high recall/F1 scores of up to 99%, but these models underperform in practical scenarios, particularly when assessed on entire codebases rather than just the fixing commit. This paper introduces Real-Vul, a comprehensive dataset representing real-world scenarios for evaluating vulnerability detection models. Evaluating DeepWukong, LineVul, ReVeal, and IVDetect shows a significant drop in performance, with precision decreasing by up to 95 percentage points and F1 scores by up to 91 points. Furthermore, Model performance fluctuates based on vulnerability characteristics, with better F1 scores for information leaks or code injection than for path resolution or predictable return values. The results highlight a significant performance gap that needs addressing before deploying deep learning-based vulnerability detection in practical settings. Overfitting is identified as a key issue, and an augmentation technique is proposed, potentially improving performance by up to 30%. Contributions include a dataset creation approach for better model evaluation, Real-Vul dataset, and empirical evidence of deep learning models struggling in real-world settings.

==> datasets_models.tex <==
\section{Datasets and Models used in the study}

\subsection{Datasets}
\textbf{SARD:} The Software Assurance Reference Dataset (SARD) \cite{SARD} contains a vast number of artificially produced security vulnerabilities. It has been frequently used by several research works \cite{cheng2021deepwukong}, \cite{li2018vuldeepecker} to assess the effectiveness of vulnerability detection methods. Because a program may have numerous types of vulnerabilities, each program in the SARD collection corresponds to one or more CWE IDs. The statements in the SARD programs are already labeled as good (statements without vulnerabilities), bad (statements with vulnerabilities), or mixed (statements containing vulnerabilities and their fixes). The SARD dataset contains 102,696 vulnerable programs and 1,408 \nonvulnerable programs.


\textbf{Big-Vul:} The Big-Vul dataset \cite{fan2020ac} is collected from 348 open-source Github projects, which includes 91 different CWEs from 2002 to 2019. It contains a total of 188,636 C/C++ functions, of which 10,900 are vulnerable functions, and 44,603 are vulnerable lines.  They browsed the public Common Vulnerabilities and Exposures (CVE) database and CVE-related source code repositories to acquire vulnerability information such as CVE IDs, severity rankings, and summaries. They chose CVE entries with reference URLs to publicly available Git repositories. The code changes before and after resolving a vulnerability were extracted for each relevant commit, and the vulnerable version of the function was finally obtained. A significant amount of manual effort has also been spent to verify the dataset's quality. 


\subsection{Models}
\label{Models}
\textbf{Deepwukong:} Deepwukong \cite{cheng2021deepwukong} is a graph-level vulnerability detection model. DeepWukong constructs a Program Dependence Graph (PDG) utilizing information from the control and data-flow graphs throughout the training phase. The program's slices (or XFGs) are then formed by traversing the PDG forward and backward from a program point of interest until a fixed point is reached, thereby maintaining both the data and control flow. Variables in the program are normalized using their canonical form. The Doc2Vec model \cite{le2014distributed}  is used to transform the tokens in the source code program into vector form. The Graph Neural Network's inputs are divided into two types: structured information and unstructured information. The structured information comprises node and edge data, while the unstructured information comprises vector representation of the code tokens from the source code program. The inputs are then fed into a GNN model, which produces a well-trained GNN model. In the detection phase, the control and data-flow graph information are extracted from the target program. The program slices are generated from the PDG. The tokens are normalized to their canonical form, and vectors for the tokens are generated from the trained Doc2Vec model. Both the graph information and the vectors of the tokens are then fed into the well-trained graph vulnerability detection models from the previous stage, and the graph is classified as vulnerable or \nonvulnerable. 

\textbf{LineVUL:} LineVUL is a line-level vulnerability detection model. CodeBERT \cite{feng2020codebert}, a BERT-based model that is trained on a huge corpus of publicly available open-source GitHub repositories is used to generate the embeddings of the source code tokens. First, lineVUL performs function-level classification. It encodes the subword-tokenized function using word and positional encoding to build an embedding vector for each word and its location in the function. The vector is then passed into the CodeBERT architecture, which comprises 12 Transformer encoder blocks stacked on top of each other. Each encoder is made up of a multi-head self-attention layer and a feed-forward neural network that is fully connected. Finally, the output vector is passed into a single linear layer for binary classification of the given function. To localize the vulnerable lines, the functions that are predicted as vulnerable are filtered out from the \nonvulnerable functions. The scores from the self-attention layers of CodeBERT are used to find the vulnerable lines. The tokens that have higher weightage for the prediction are assumed to be vulnerable tokens. So the self-attention scores from all the transformer encoder blocks are extracted, which are then used to assign line scores for each source code line. The source code lines are then ranked in descending order based on the scores, with the most likely vulnerable line at the top and the least likely vulnerable line at the bottom.  



==> tables/RQ1.tex <==
\bgroup

\begin{table}[tb!]
\caption{Replication results of LineVUL and Deepwukong.}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Dataset / Model} & \textbf{Acc {[}\%{]}} & \textbf{Prec {[}\%{]}} & \textbf{Recall {[}\%{]}} & \textbf{F1 {[}\%{]}} \\ \hline
    SARD / Deepwukong        & 98.00                        & 87.00                         & 98.00                      & 93.00                        \\ \hline
    BigVUL / LineVUL         & 96.00                        & 96.00                         & 84.00                      & 90.00                       \\ \hline
\end{tabular}
\label{table:table_rq1}
\end{table}
\egroup


==> tables/RQ2_deepwukong.tex <==
\bgroup
\begin{table}[htb]
\caption{Results of Deepwukong model trained and tested using the imbalanced dataset}
\label{table:table_rq2_deepwukong}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Projects} & \textbf{Acc {[}\%{]}} & \textbf{Prec {[}\%{]}} & \textbf{Recall {[}\%{]}} & \textbf{F1 {[}\%{]}} \\ \hline
Chrome           & 99.87                     & 0.00                       & 0.00                    & 0.00                         \\ \hline
Linux            & 99.94                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
ImageMagick      & 97.81                     & 13.72                      & 5.08                    & 7.42                      \\ \hline
Tcpdump          & 97.58                     & 7.24                       & 8.92                    & 8.00                         \\ \hline
Openssl          & 99.28                     & 0.80                        & 0.45                    & 0.58                      \\ \hline
Kerberos         & 99.43                     & 49.66                      & 28.4                    & 36.14                     \\ \hline
Php              & 99.96                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Jasper           & 96.97                     & 41.72                      & 27.88                   & 33.42                         \\ \hline
FFmpeg           & 99.81                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Qemu             & 99.95                     & 1.69                       & 1.85                    & 1.76                        \\ \hline
\textbf{Mean}           & \textbf{99.06}                        & \textbf{11.48}                         & \textbf{7.25}                      & \textbf{8.73}                       \\ \hline
% \textbf{Median}           & \textbf{99.62}                        & \textbf{1.24}                         & \textbf{1.15}                      & \textbf{1.17}                       \\ \hline
% \textbf{Min}           & \textbf{96.97}                        & \textbf{0.00}                         & \textbf{0.00}                      & \textbf{0.00}                       \\ \hline
% \textbf{Max}           & \textbf{99.96}                        & \textbf{49.66}                         & \textbf{28.40}                      & \textbf{36.14}                       \\ \hline
\end{tabular}
\end{table}
\egroup

==> tables/RQ2_linevul.tex <==
\bgroup
\begin{table}[htb]
\caption{Results of LineVUL model trained and tested using the imbalanced dataset}
\label{table:table_rq2_linevul}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Projects} & \textbf{Acc {[}\%{]}} & \textbf{Prec {[}\%{]}} & \textbf{Recall {[}\%{]}} & \textbf{F1 {[}\%{]}} \\ \hline
Chrome           & 99.79                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Linux            & 99.93                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
ImageMagick      & 99.36                     & 0.00                          & 0.00                       & 0.00                      \\ \hline
Tcpdump          & 94.64                     & 16.66                         & 55.88                      & 25.67                     \\ \hline
Openssl          & 99.77                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Kerberos         & 98.34                     & 16.05                         & 56.41                      & 25.00                     \\ \hline
PHP              & 99.92                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Jasper           & 97.13                     & 56.25                         & 69.23                      & 62.06                         \\ \hline
FFmpeg           & 99.94                     & 0.00                          & 0.00                       & 0.00                         \\ \hline
Qemu             & 99.95                     & 0.00                          & 0.00                       & 0.00                        \\ \hline
\textbf{Mean}           & \textbf{98.87}                        & \textbf{8.89}                         & \textbf{18.15}                      & \textbf{11.27 }                       \\ \hline
% \textbf{Median}           & \textbf{99.78}                        & \textbf{0.00}                         & \textbf{0.00}                      & \textbf{0.00}                       \\ \hline
% \textbf{Min}           & \textbf{94.64}                        & \textbf{0.00}                         & \textbf{0.00}                      & \textbf{0.00}                       \\ \hline
% \textbf{Max}           & \textbf{99.95}                        & \textbf{56.25}                         & \textbf{69.23}                      & \textbf{62.06}                       \\ \hline
\end{tabular}
\end{table}
\egroup

==> tables/RQ3_deepwukong.tex <==
\bgroup
\begin{table}[htb]
\caption{Results of Deepwukong model trained using the balanced dataset and tested using the imbalanced dataset}
\label{table:table_rq3_deepwukong}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Projects} & \textbf{Acc {[}\%{]}} & \textbf{Prec {[}\%{]}} & \textbf{Recall {[}\%{]}} & \textbf{F1 {[}\%{]}} \\ \hline
Chrome           & 92.13                     & 0.29                      & 18.66                    & 0.57                         \\ \hline
Linux            & 94.37                     & 0.13                        & 14.29                       & 0.26                        \\ \hline
ImageMagick      & 90.62                     & 8.38                      & 44.71                    & 14.12                      \\ \hline
Tcpdump          & 84.17                     & 1.73                       & 22.32                    & 3.21                         \\ \hline
Openssl          & 91.77                     & 1.51                        & 26.48                    & 2.87                      \\ \hline
Kerberos         & 92.12                     & 6.04                      & 88.63                    & 11.30                     \\ \hline
Php              & 84.67                     & 0.03                          & 12.12                       & 0.06                         \\ \hline
Jasper           & 80.00                     & 9.65                      & 75.96                   & 17.13                         \\ \hline
FFmpeg           & 93.40                     & 0.27                          & 10.53                      & 0.52                         \\ \hline
Qemu             & 85.58                     & 0.03                      & 25.92                   & 0.07                       \\ \hline
\textbf{Mean}           & \textbf{88.88}                        & \textbf{2.80}                         & \textbf{33.96}                      & \textbf{5.01}                       \\ \hline
% \textbf{Median}           & \textbf{91.19}                        & \textbf{0.90}                         & \textbf{24.12}                      & \textbf{1.72}                       \\ \hline
% \textbf{Min}           & \textbf{80.00}                        & \textbf{0.03}                         & \textbf{10.53}                      & \textbf{0.06}                       \\ \hline
% \textbf{Max}           & \textbf{94.37}                        & \textbf{9.65}                         & \textbf{88.63}                      & \textbf{17.13}                       \\ \hline
\end{tabular}
\end{table}
\egroup

==> tables/RQ3_linevul.tex <==
\bgroup
\begin{table}[htb]
\caption{Results of LineVUL model trained using the balanced dataset and tested using the imbalanced dataset}
\label{table:table_rq3_linevul}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Projects} & \textbf{Acc {[}\%{]}} & \textbf{Prec {[}\%{]}} & \textbf{Recall {[}\%{]}} & \textbf{F1 {[}\%{]}} \\ \hline
Chrome           & 88.61                        & 1.65                          & 92.16                      & 3.25                         \\ \hline
Linux      & 64.29                        & 0.17                          & 98.15                      & 0.35                         \\ \hline
ImageMagick      & 99.36                        & 0.00                          & 0.00                      & 0.00                         \\ \hline
Tcpdump          & 98.34                        & 0.00                         & 0.00                      & 0.00                        \\ \hline
OpenSSL          & 0.57                        & 0.22                          & 100                      & 0.45                         \\ \hline
Kerberos         & 36.13                        & 0.66                          & 87.17                      & 1.30                         \\ \hline
PHP         & 74.01                        & 0.29                          & 100                      & 0.58                         \\ \hline
Jasper           & 96.61                        & 0.00                          & 0.00                      & 0.00                         \\ \hline
FFmpeg           & 31.76                        & 0.07                          & 94.44                      & 0.14                        \\ \hline
Qemu             & 99.95                         & 0.00                          & 0.00                      & 0.00                         \\ \hline
\textbf{Mean}           & \textbf{68.96}                        & \textbf{0.30}                         & \textbf{57.19}                      & \textbf{0.60}                       \\ \hline
% \textbf{Median}           & \textbf{81.31}                        & \textbf{0.12}                         & \textbf{89.66}                      & \textbf{0.24}    \\ \hline
% \textbf{Min}           & \textbf{0.57}                        & \textbf{0}                         & \textbf{0}                      & \textbf{0}                       \\ \hline
% \textbf{Max}           & \textbf{99.95}                        & \textbf{0.66}                         & \textbf{100}                      & \textbf{1.3}                       \\ \hline
\end{tabular}
\end{table}
\egroup


==> tables/train_test_splits.tex <==
\bgroup
\begin{table}[htb]
\caption{The train and test dataset splits of our datasets}
\label{table:table_train_test_split}
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Project} & \textbf{Train Dataset Period} & \textbf{Test Dataset Period} \\ \hline
Chrome           & 2011 - 2017                   & 2018 - 2019                  \\ \hline
ImageMagick      & 2016 - 2018                   & 2019                    \\ \hline
Kerberos         & 2012 - 2015                   & 2016 - 2018                  \\ \hline
OpenSSL          & 2013 - 2016                   & 2017 - 2019                  \\ \hline
Tcpdump          & 2014 - 2017                   & 2019                         \\ \hline
Php-Src          & 2013 - 2016                   & 2017 - 2019                  \\ \hline
Qemu             & 2013 - 2017                   & 2018 - 2019                  \\ \hline
Ghostscript      & 2014 - 2017                   & 2018 - 2019                  \\ \hline
FFmpeg           & 2013 - 2017                   & 2018 - 2019                  \\ \hline
Jasper           & 2017                          & 2018                         \\ \hline
\end{tabular}
\end{table}
\egroup
